HLT@SUDA at SemEval 2019 Task 1: UCCA Graph Parsing as Constituent Tree Parsing

This paper describes a simple UCCA semantic graph parsing approach. The key idea is to convert a UCCA semantic graph into a constituent tree, in which extra labels are deliberately designed to mark remote edges and discontinuous nodes for future recovery. In this way, we can make use of existing syntactic parsing techniques. Based on the data statistics, we recover discontinuous nodes directly according to the output labels of the constituent parser and use a biaffine classification model to recover the more complex remote edges. The classification model and the constituent parser are simultaneously trained under the multi-task learning framework. We use the multilingual BERT as extra features in the open tracks. Our system ranks the first place in the six English/German closed/open tracks among seven participating systems. For the seventh cross-lingual track, where there is little training data for French, we propose a language embedding approach to utilize English and German training data, and our result ranks the second place.

==> content/not-used/approach-pred.tex <==
\subsection{Evaluation Phase}

After getting predicted constituency trees using the trained model, we need to restore all of them to UCCA scheme. To restore the graphs, we should reverse previous steps of conversion. That is, we first move labels from nodes to edges. Then restore all discontinuities in the initiative converted graphs using a rule-based approach. Finally we use the previous jointly trained biaffine classifier to restore all remote edges.

\textbf{Restore discontinuities.} For all nodes in a UCCA graph, if a edge has \textbf{\textit{-down}} suffix in its label, we just need to change the parent of the edge to the parent of origin parent.


==> content/not-used/approach-train.tex <==
\subsection{Multi-task Training}

It is natural to employ multi-task learning framework to train three parts of the parser jointly.  Given input tokens, a bidirectional LSTM is set at the bottom as shared encoder to obtain context-sensitive forward and backward encodings for each position $i$ , denoted by $f_i$ and $b_i$, respectively. Our representation of the $span(i,j)$ is the concatenation the vector differences $f_j − f_i$ and $b_i − b_j$. With span vectors feed in, we then use the representations to train the constituency parser and remote classifier jointly. 

\textbf{Top-Down Parsing} We adopt a greedy top-down inference algorithm used in minimal span-based parser to train the  constituency parser. That is, given a span, we independently assign it a label and pick a split point, then repeat this process for the left and right subspans. To obtain the loss for a given training example, we trace out the actions corresponding to the gold tree and accumulate the penalties of label and split points. Here we denote it as $loss_{topdown}$.

\textbf{Remote classifier} 

By combining the above two loss functions, the final loss is $loss_{topdown}+loss_{remote}$, so we have achieved joint training for them.

==> image/fig.tex <==
% File acl2017.tex
%
%% Based on the style files for ACL-2015, with some improvements
%%  taken from the NAACL-2016 style
%% Based on the style files for ACL-2014, which were, in turn,
%% based on ACL-2013, ACL-2012, ACL-2011, ACL-2010, ACL-IJCNLP-2009,
%% EACL-2009, IJCNLP-2008...
%% Based on the style files for EACL 2006 by
%%e.agirre@ehu.es or Sergi.Balari@uab.es
%% and that of ACL 08 by Joakim Nivre and Noah Smith

% \documentclass[border=0.0mm]{standalone}

% \usepackage{times}
% \usepackage{latexsym}
% \usepackage{CJKutf8}

% \usepackage{url}

% \usepackage{helvet}
% \usepackage{courier}
% \usepackage{subfigure}
% \usepackage{multirow}
% \usepackage{subfigure}
% \usepackage{arydshln}
% \usepackage{color}
% \usepackage{amsmath,amssymb,bm}
% \usepackage{algorithm}
% \usepackage{algorithmic}
% \usepackage[american]{babel}
% \usepackage[c]{esvect}
% %\usepackage{hyphenat}
% \usepackage{graphicx}
% \usepackage{tikz}
% \usepackage{tikz-dependency}
% \usepackage{pgfplots}
% \usetikzlibrary{patterns,shapes,snakes,calendar,matrix,backgrounds,folding,arrows,arrows.meta}
% \usepackage{footnote}


\tikzset{
wordnode/.style = {circle,fill=black,inner sep=0,minimum size=4pt},
arc/.style = {draw,  -latex'},
decision/.style = {diamond, draw, fill=blue!20,
  text width=4.5em, text badly centered, node distance=3cm, inner sep=0pt},
block/.style = {rectangle, draw, fill=blue!20,
  text width=3em, text centered, rounded corners, minimum height=4em},
textdata/.style = {rectangle,
  text width=3em, text centered, minimum height=4em},
procedure/.style = {rectangle, draw, fill=blue!20,
  text width=3.5em, text centered,  minimum height=3em,  minimum width=3em},
line/.style = {draw,very thick,  -latex'},
line1/.style = {draw, thick, dashed},
compose/.style = {rectangle, draw, fill=none, rounded corners, blue, thick},
cloud/.style = {draw, ellipse,fill=red!20, node distance=3cm,
  minimum height=2em},
subroutine/.style = {draw,rectangle split,
  rectangle split parts=3,minimum height=1cm,
  rectangle split part fill={red!50, green!50, blue!20, yellow!50}},
connector/.style = {draw,circle,node distance=3cm,fill=yellow!20},
data/.style = {draw, trapezium, text width=3em, align=center, fill=olive!20, trapezium left angle=75pt, trapezium right angle=105, trapezium stretches = true, minimum height=3em, minimum width = 3em},
mytrap/.style={trapezium, trapezium angle=67.5, draw, inner ysep=5pt, outer sep=0pt,  minimum height=1.81mm, minimum width=0pt}
}

\definecolor{a1c}{rgb}{0.00,0.00,1}
\definecolor{a2c}{rgb}{0.30,0.00,0.70}
\definecolor{a3c}{rgb}{0.00,0.50,0.50}
\definecolor{a4c}{rgb}{0.70,0.00,0.70}
\definecolor{a5c}{rgb}{1.00,0.00,0.00}
\definecolor{a6c}{rgb}{0.00,1.00,0.00}

\definecolor{redi}{RGB}{255,38,0}
\definecolor{redii}{RGB}{200,50,0}
\definecolor{yellowi}{RGB}{255,251,0}
\definecolor{bluei}{RGB}{0,150,255}
\definecolor{blueii}{RGB}{135,247,210}
\definecolor{blueiii}{RGB}{91,205,250}
\definecolor{blueiv}{RGB}{115,244,253}
\definecolor{bluev}{RGB}{1,58,215}
\definecolor{orangei}{RGB}{240,143,50}
\definecolor{yellowii}{RGB}{222,247,100}
\definecolor{greeni}{RGB}{166,247,166}


\depstyle{stanford1}{edge style = {thick, red}, edge height = 0.3cm, edge horizontal padding=9.0pt, label style={thick, draw=white, text=red, fill=white, rotate = 0}}
\depstyle{stanford2}{edge style = {thick, red}, edge height = 0.6cm, edge horizontal padding=7.2pt, label style={thick, draw=white, text=red, fill=white, rotate = 0}}
\depstyle{stanford3}{edge style = {thick, red}, edge height = 0.9cm, edge horizontal padding=5.4pt, label style={thick, draw=white, text=red, fill=white, rotate = 0}}
\depstyle{stanford4}{edge style = {thick, red}, edge height = 1.6cm, edge horizontal padding=3.6pt, label style={thick, draw=white, text=red, fill=white, rotate = 0}}
\depstyle{stanford5}{edge style = {thick, red}, edge height = 1.9cm, edge horizontal padding=1.8pt, label style={thick, draw=white, text=red, fill=white, rotate = 0}}
\depstyle{stanford6}{edge style = {thick, red}, edge height = 2.5cm, edge horizontal padding=0.0pt, label style={thick, draw=white, text=red, fill=white, rotate = 0}}
\depstyle{stanford7}{edge style = {thick, red}, edge height = 1.5cm, edge horizontal padding=0.0pt, label style={thick, draw=white, text=red, fill=white, rotate = 0}}




%\aclfinalcopy % Uncomment this line for the final submission
%\def\aclpaperid{***} %  Enter the acl Paper ID here

%\setlength\titlebox{5cm}
% You can expand the titlebox if you need extra space
% to show all the authors. Please do not make the titlebox
% smaller than 5cm (the original size); we will check this
% in the camera-ready version and ask you to change it back.




%\author{First Author \\
%  Affiliation / Address line 1 \\
%  Affiliation / Address line 2 \\
%  Affiliation / Address line 3 \\
%  {\tt email@domain} \\\And
%  Second Author \\
%  Affiliation / Address line 1 \\
%  Affiliation / Address line 2 \\
%  Affiliation / Address line 3 \\
%  {\tt email@domain} \\}

%\thispagestyle{empty}
% \begin{document}
% \begin{CJK}{UTF8}{gbsn}


% \begin{small}
% \renewcommand\arraystretch{0.7}
% \setlength{\tabcolsep}{3pt}
\begin{figure*}[tb]
\begin{center}
\begin{small}
\begin{tikzpicture}[node distance = 0.1cm, auto]
\definecolor{mycolor}{RGB}{228, 198, 208}
\definecolor{mycolor2}{RGB}{161, 175, 201}
\definecolor{mycolor3}{RGB}{135, 186, 191}

\node [inner sep=0pt] (lstm_orig) {};

\node [rectangle, above = 2 em of lstm_orig, node distance = 15em, rounded corners, draw, fill=blue!40, text centered, minimum width=2.5em, minimum height=1.5em] (a1) {};

%\node [rectangle, above = 2 em of pat_orig, node distance = 30em, rounded corners, draw, fill=blue!40, text centered, minimum width=2.5em, minimum height=1.5em] (xxxx1) {};

%\node [rectangle, above = 2 em of treelstm_orig, node distance = 15em, rounded corners, draw, fill=blue!40, text centered, minimum width=3.5em, minimum height=1.5em] (xxxx2) {};

\node [inner sep=0pt, left of=a1, node distance = 3em] (a0) {\bf ...};
\node [rectangle, rounded corners, draw, fill=blue!40, text centered, minimum width=2.5em, minimum height=1.5em, right of = a1, node distance = 4em] (a2) {};

\node [inner sep=0pt, right of=a2, node distance = 3em] (a3) {\bf ...};

\node [rectangle, rounded corners, draw, fill=blue!40, text centered, minimum width=2.5em, minimum height=1.5em, right of = a3, node distance = 3em] (a4) {};
\node [inner sep=0pt, right of=a4, node distance = 3em] (a5) {\bf ...};

\node [rectangle, above of = a1, node distance = 3em, rounded corners, draw, fill=blue!40, text centered, minimum width=2.5em, minimum height=1.5em] (l1) {};
\node [inner sep=0pt, above of=a0, node distance = 3em] (l0) {\bf ...};
\node [rectangle, above of = a2, node distance = 3em, rounded corners, draw, fill=blue!40, text centered, minimum width=2.5em, minimum height=1.5em] (l2) {};
\node [inner sep=0pt, above of=a3, node distance = 3em] (l3) {\bf ...};
\node [rectangle, above of = a4, node distance = 3em, rounded corners, draw, fill=blue!40, text centered, minimum width=2.5em, minimum height=1.5em] (l4) {};
\node [inner sep=0pt, above of = a5, node distance = 3em] (l5) {\bf ...};

% \node [rectangle, right of = x, node distance = 30em, rounded corners, draw, fill=blue!40, text centered, minimum width=3.5em, minimum height=1.5em] (l) {};



\node [inner sep=0pt, below of=a1, node distance = 2em] (z1) {};
\path [draw, thick, ->, >=stealth'] (z1) to [out=90,in=-90] (a1);

\node [inner sep=0pt, below of=a2, node distance = 2em] (z2) {};
\path [draw, thick, ->, >=stealth'] (z2) to [out=90,in=-90] (a2);

\node [inner sep=0pt, below of=a4, node distance = 2em] (z3) {};
\path [draw, thick, ->, >=stealth'] (z3) to [out=90,in=-90] (a4);

% $\bf h_{j}$

% 第一层LSTM node之间的线
\path [draw, thick, <->, >=stealth'] (a1) to [out=60,in=120]  (a2);

\node [inner sep=0pt, above left = 0.5em and 0.1em of a3, node distance = 0.5em] (a3_above_left) {};
\path [draw, thick, <->, >=stealth'] (a2) to [out=60,in=120]  (a3_above_left);

\node [inner sep=0pt, above right = 0.5em and 0.1em of a3, node distance = 0.5em] (a3_above_right) {};
\path [draw, thick, <->, >=stealth'] (a3_above_right) to [out=60,in=120]  (a4);

\node [inner sep=0pt, above of=a5, node distance = 0.5em] (a5_above){};
\path [draw, thick, <->, >=stealth'] (a4) to [out=60,in=120]  (a5_above);

\node [inner sep=0pt, above of=a0, node distance = 0.5em] (above_a0) {};
\path [draw, thick, <->, >=stealth'] (above_a0) to [out=60,in=120]  (a1);


% 第二层LSTM node之间的线
% \path [draw, thick, <->, >=stealth'] (l1) to [out=40,in=140]  (l2);
% \node [inner sep=0pt, right of=l2, node distance = 3em] (l30) {};
% \node [inner sep=0pt, above of=l30, node distance = 0.6em] (l31) {};
% \path [draw, thick, <->, >=stealth'] (l2) to [out=60,in=120]  (l31);

% \node [inner sep=0pt, right of=l31, node distance = 2em] (l32) {};
% \path [draw, thick, <->, >=stealth'] (l32) to [out=60,in=120]  (l4);

% \node [inner sep=0pt, right of=l31, node distance = 8em] (l33) {};
% \path [draw, thick, <->, >=stealth'] (l4) to [out=60,in=120]  (l33);

% \node [inner sep=0pt, above of=l0, node distance = 0.5em] (above_l0) {};
% \path [draw, thick, <->, >=stealth'] (above_l0) to [out=60,in=120]  (l1);

\path [draw, thick, <->, >=stealth'] (l1) to [out=60,in=120]  (l2);

\node [inner sep=0pt, above left = 0.5em and 0.1em of l3, node distance = 0.5em] (l3_above_left) {};
\path [draw, thick, <->, >=stealth'] (l2) to [out=60,in=120]  (l3_above_left);

\node [inner sep=0pt, above right = 0.5em and 0.1em of l3, node distance = 0.5em] (l3_above_right) {};
\path [draw, thick, <->, >=stealth'] (l3_above_right) to [out=60,in=120]  (l4);

\node [inner sep=0pt, above of=l5, node distance = 0.5em] (l5_above){};
\path [draw, thick, <->, >=stealth'] (l4) to [out=60,in=120]  (l5_above);

\node [inner sep=0pt, above of=l0, node distance = 0.5em] (above_l0) {};
\path [draw, thick, <->, >=stealth'] (above_l0) to [out=60,in=120]  (l1);


\path [draw, thick, ->, >=stealth'] (a1) to [out=90,in=-90]  (l1);
\path [draw, thick, ->, >=stealth'] (a2) to [out=90,in=-90]  (l2);
\path [draw, thick, ->, >=stealth'] (a4) to [out=90,in=-90]  (l4);

% 两层LSTM外面的大框
\node [compose, fill = blue!20, blue, opacity=.4, above right = 1.3em and -3.9em  of lstm_orig, minimum height = 6.5em,  minimum width = 18em] (lstm_out_rect){};
\node [inner sep=0pt, left of =lstm_out_rect, node distance = 13em] (lstm_text) { BiSeqLSTM };
\node [inner sep=0pt, below  of=lstm_text, node distance = 1em] (lstm_text2) { (two layers)};


\node [rectangle, rounded corners, draw, fill=blue!20, text centered, minimum width=3.5em, minimum height=1.5em, above of = a1, node distance = 10em] (mlp_d) {};

\node [inner sep=0pt, left = 0.2em of mlp_d] (mlp_d_text){ $\texttt{MLP}^{\textup{D}}$};

\node [rectangle, rounded corners, draw, fill=blue!20, text centered, minimum width=3.5em, minimum height=1.5em, above of = a4, node distance = 10em] (mlp_h) {};

\node [inner sep=0pt, left = 0.2em of mlp_h] (mlp_h_text){ $\texttt{MLP}^{\textup{H}}$};

%\node [inner sep=0pt, minimum width=3.5em, minimum height=1.5em, right of = middle_above_lstm, node distance = 2.5em] (b2) {};

%\node [inner sep=0pt, above of=a4, node distance = 8em] (b3) {};


\node [inner sep=0pt,  above left = 1.4em and -0.6em of l4] (h_seq_j) {$\mathbf{h}_j^{seq}$};
\node [inner sep=0pt,  above left = 1.4em and -0.6em of l1] (h_seq_i) {$\mathbf{h}_i^{seq}$};


\path [draw, thick, ->, >=stealth'] (l1) to [out=90,in=-90]  (mlp_d);

\path [draw, thick, ->, >=stealth'] (l4) to [out=90,in=-90]  (mlp_h);

\node [inner sep=0pt, above left = 0.3em and -1.2em of mlp_d] (ri) {$\mathbf{r}_{i,i\leftarrow j}^{\textup D}$};
\node [inner sep=0pt, above left = 0.3em and -1.2em of mlp_h] (rj) {$\mathbf{r}_{j,i\leftarrow j}^{\textup H}$};

\node [inner sep=0pt, above of=lstm_out_rect, node distance = 8em] (middle_above_lstm) {};

\node [rectangle, rounded corners, draw, fill=mycolor2, text centered, minimum width=3.5em, minimum height=1.5em, above of = middle_above_lstm, node distance = 6em] (biaffine) {};
%
\node [inner sep=0pt, left of = biaffine, node distance = 4.0em] (biaffine_text){Biaffine};


\node [inner sep=0pt, above of = biaffine, node distance = 4.0em] (score) {$\texttt{score}(i \leftarrow j)$};

\path [draw, thick, ->, >=stealth'] (biaffine) to [out=90,in=-90] (score) ;

\path [draw, thick, ->, >=stealth'] (mlp_d) to [out=90,in=-135]  (biaffine);

\path [draw, thick, ->, >=stealth'] (mlp_h) to [out=90,in=-45]  (biaffine);


%%% Pattern embedding part %%%
\node [inner sep=0pt, above left = 22em and 13em of lstm_orig] (pat_orig) {};


\node [inner sep=0pt, below of = pat_orig] (pat1) { consistent:  $i  \leftarrow j$};
\node [inner sep=0pt, below of=pat1, node distance = 1.5em] (pat2) { grand:  $i  \leftarrow k  \leftarrow j$};
\node [inner sep=0pt, below of=pat2, node distance = 1.5em] (pat3) { sibling:  $i  \leftarrow k  \rightarrow j$};
\node [inner sep=0pt, below of=pat3, node distance = 1.5em] (pat4) { reverse:  $i  \rightarrow j$};
\node [inner sep=0pt, below of=pat4, node distance = 1.5em] (pat5) { reverse grand:  $i  \rightarrow k  \rightarrow j$};
\node [inner sep=0pt, below of=pat5, node distance = 1.5em] (pat6) { else: $\{ 3;4-5;6;\ge7\}$}; 

\node [compose, color=black, fill = white, opacity=.4,  below of = pat3
, minimum height = 10em,  minimum width = 12em, node distance=1em]   (pattern_out_rect){};

% \node [inner sep=0pt, fill=black, below left = 1.0em and 0em of b1] (null) {};
% \path [draw, thick, ->, >=stealth'] (null) to [out=80,in=-150]  (b1);
% \path [draw, thick, ->, >=stealth'] (null) to [out=0,in=-150]  (b5);
% \node [inner sep=0pt, above right = 8 em and 6 em of a5, node distance = 10em] (d0) {};

\node [inner sep=0pt,  below right = 1.5em and -4.0em of pat6] (pat_emb) {$\mathbf{e}^{p_{i \leftarrow j}}$};

\node [rectangle, rounded corners, draw, fill=mycolor, text centered, minimum width=3.5em, minimum height=1.5em, below = 3.5em of pat6] (r_pat) {};
\node [inner sep=0pt, above right = -0.2em and 0.5em of r_pat] (r_pat_text) {$\mathbf{r}^{pat}_{i \leftarrow j}$};

\node [inner sep=0pt,  below = 2em of r_pat] (pat_label_emb) {$\mathbf{e}^{l_i} \oplus \mathbf{e}^{l_j} \oplus  \mathbf{e}^{l_a}$};
\node [inner sep=0pt, above = 0.1em of pat_label_emb] (pat_label_emb_above) {};




\path [draw, thick, ->, >=stealth'] (pat_label_emb_above) to [out=90,in=-90]  (r_pat);
\path [draw, thick, ->, >=stealth'] (pattern_out_rect) to [out=-90,in=90]  (r_pat);
\path [draw, thick, ->, >=stealth'] (r_pat) to [out=0,in=-150]  (mlp_d);
\path [draw, thick, ->, >=stealth'] (r_pat) to [out=0,in=-150]  (mlp_h);




%%% TreeLSTM part %%%

\node [inner sep=0pt, above right = 22em and 23em of lstm_orig] (treelstm_orig) {};

\node [rectangle, rounded corners, draw, fill=mycolor3, text centered, minimum width=3.5em, minimum height=1.5em, below = 0.1em of treelstm_orig] (w_a) { $w_a$};
%d1

% \bf ${\text {r}}^{\text {tree}}_{\text {i} \leftarrow \text {j}}$

\node [rectangle, rounded corners, draw, fill=mycolor3, text centered, minimum width=3.5em, minimum height=1.5em, below left = 2em and -0.1em of w_a] (w_i) {\bf $w_i$};
%d2

\node [rectangle, rounded corners, draw, fill=mycolor3, text centered, minimum width=3.5em, minimum height=1.5em, right = 3em of w_i] (w_k) {};
%d3

\node [rectangle, rounded corners, draw, fill=mycolor3, text centered, minimum width=3.5em, minimum height=1.5em, below = 2em of w_k, node distance = 3em] (w_j) {\bf $w_j$};
%d5

\node [rectangle, rounded corners, draw, fill=mycolor, text centered, minimum width=3.5em, minimum height=1.5em, right = 33em of r_pat, node distance = 5em] (r_tree) {};
%\path [draw, thick, ->, >=stealth', mycolor]  (d11) to [out=190, in=-70]  (b5);
\node [inner sep=0pt,  above left = -0.1em and 0.5em of r_tree] (r_tree_text) {$\mathbf{r}^{tree}_{i \leftarrow j}$};


\path [draw, thick, ->, >=stealth'] (r_tree) to [out=180,in=-30]  (mlp_d);
\path [draw, thick, ->, >=stealth'] (r_tree) to [out=180,in=-30]  (mlp_h);

\path [draw, thick, ->, >=stealth', dashed] (w_i) to [out=30,in=-100]  (w_a);
\path [draw, thick, ->, >=stealth', dashed, blue] (w_a) to [out=-135,in=70]  (w_i);

\path [draw, thick, ->, >=stealth', dashed] (w_k) to [out=150,in=-80]  (w_a);
\path [draw, thick, ->, >=stealth', dashed, blue] (w_a) to [out=-45,in=110]  (w_k);

\path [draw, thick, ->, >=stealth', dashed] (w_j) to [out=120,in=-120]  (w_k);
\path [draw, thick, ->, >=stealth', dashed, blue] (w_k) to [out=-60,in=60]  (w_j);


\path [draw, thick, ->, >=stealth', dashed] (w_a) to [out=5,in=5]  (r_tree);
\path [draw, thick, ->, >=stealth', dashed, blue] (w_i) to [out=-90,in=120]  (r_tree);
\path [draw, thick, ->, >=stealth', dashed, blue] (w_j) to [out=-100,in=60]  (r_tree);





\node [inner sep=0pt,  below left = 0.1em and -0.1em of w_i] (h_i_tree) {$\mathbf{h}_i^{\downarrow}$};
\node [inner sep=0pt,  below left = 0.1em and 0.1em of w_j] (h_j_tree) {$\mathbf{h}_j^{\downarrow}$};
\node [inner sep=0pt,  above right = 0.1em and 0.1em of w_a] (h_a_tree) {$\mathbf{h}_a^{\uparrow}$};

\end{tikzpicture}
\caption{Computation of $\texttt{score}(i \leftarrow j)$ in our proposed conversion approaches. Without the source-side tree $\mathbf{d}^{src}$, the baseline uses the basic $\mathbf{r}_{i}^{\textup D}$ and $\mathbf{r}_{j}^{\textup H}$ (instead of $\mathbf{r}_{i,i \leftarrow j}^{\textup D}$ and $\mathbf{r}_{j,i \leftarrow j}^{\textup H}$).}\label{fig:approach}
\end{small}
\end{center}
\end{figure*}
        
%\end{small}


% \end{CJK}
% \end{document}

